DAT: Data Architecture Modeling Tool for Data-Driven Applications

Data is the key to success for any Data-Driven Organization, and managing it is considered the most challenging task. Data Architecture (DA) focuses on describing, collecting, storing, processing, and analyzing the data to meet business needs. In this tool demo paper, we present the DAT, a model-driven engineering tool enabling data architects, data engineers, and other stakeholders to describe how data flows through the system and provides a blueprint for managing data that saves time and effort dedicated to Data Architectures for IoT applications. We evaluated this work by modeling five case studies, receiving expressiveness and ease of use feedback from two companies, more than six researchers, and eighteen undergraduate students from the software architecture course

==> application.tex <==
\section{Application of DAT Models to the AQSS Case Study}
\label{sec:casestudy}

This section introduces the AQSS (L'Aquila City Stree Science) case study and its DAT.


\subsection{The L'Aquila City Street Science Case Study}
\label{sec:back-NDR}
L'Aquila Street Science (AQSS) is a scientific exhibition organized by the University of L'Aquila in the context of the European Researchers Night. 
%In this event, the research community and the public are gathered together throughout the day to share their entertainment and information. This event takes place in the entire city. 
%As a real demonstrative example of what exactly happens in a part of this event, we are going to take. 
AQSS contains workshops, performances, lectures, and demonstrations in the city’s square, the main streets, and buildings. We have gotten these pieces of evidence from our experiences of organizing this event every year. First, around 25,000 visitors come to the event. Second, busiest late hours. Third, the visitor’s preferences change %(what to see and where to stay more).
based on the weather situation. Forth, it is not easy for visitors to locate activities and miss some of them. Fifth, Different entertainment events take place in different venues with limited capacity. We as a (research group) have been invited to provide a solution to improve the quality of the visiting experience. These solutions are related to parking lot control and venue crowd management. For Automated Parking Control, only two parking lots are available in the city center, with 200 and 150 parking slots, respectively. %These parking lots are created in an ad-hoc way a day prior to the event. This means that.
The visitors need to be notified about the availability in a particular parking lot and redirected accordingly to reduce the traffic congestion in the center. These parking lots are closer to the main venue where the most important event occurs. For Automated Venue Entry Management, during the AQSS event, there will be significant events in multiple indoor venues in the city center. Each of these venues has some entertainment as well as infotainment events. However, there are space limitations in each of these venues, which allows entry to only a certain number of visitors with entrance tickets at a given instant of time. % (In this work, we focus on three venues located in the city center with a seating capacity of 500 and 200 seats, respectively). This calls for services that can automatically manage the venue entry by considering the number of people inside the venue and providing real-time updates to the visitors on venue availability. 
In this paper, we are going to describe the data flow for this event by drawing the model that represents it using our DAT tool.

\subsection{The DAT model applied to the AQSS Case Study}
This section shows the DAT of the AQSS case study. From a structural point of view, Figure \ref{fig:ndr} shows the main six data nodes; Data Generation, Data Ingestion, Real-time processing, Raw Data, Batch Processing, Storage and Consuming Data. %\todo[inline]{Follow the same order you use in the figure... Data Sources, Data Ingestion, Real Time processing, Storage, etc.}
The \textit{Data Generation} node is responsible for representing the rule of generating different data formats (e.g JSON, Video) from different data sources such as(People counter, Parking mat and Camera) and transferring the data to \textit{Data Ingestion} node. It describe how data extracted from various data sources and loaded into downstream. %(responsible of making the data available to the data pipeline)., which includes identify, validate, compress, reduce the noise, and transform into a uniform data format.
After that, the data will be moved into two  nodes Raw Data and Real-Time Processing. 
The \textit{Raw Data} node is responsible for saving the data in the natives formats  using one of File System storage technologies like (HDFS) to be used as a historical data and to fed the batch Processing node. The \textit{Real-Time} and \textit{Batch Processing} nodes have similar processing functionalities, including classifying the incoming data, filtering, cleaning, and transforming to another format to be stored in different kinds of DBs to be compatible for later usage. Real-time processing works whenever the data is available to handle continuous stream data. At the same time, Batch Processing waits a specific amount of time to handle the collected data group. After that, in the \textit{Storage and Analyze} phase, the data will be stored in different kinds of databases (Relational and Column Oriented) to be ready to serve any query or any other data consumption or to be ready for any analysis. %like (diagnose, describe, predict). 
Finally, Consume the data to show the data on any presentation or provide it to be consumed for another usage. 
%\todo[inline]{the last paragraph is NOT clear. Rewrite.}
\begin{center} 
   \begin{figure*}[t!]
	\centering
	%\makebox[\textwidth]
%	{
	    	\includegraphics[width=0.9\textwidth]{figures/ndr4.png}
%	}
%
	\caption{The Data architecture of the AQSS case study - (LLA)}
	\label{fig:ndr}
    \end{figure*}
\end{center}
\begin{center} 
   \begin{figure*}[t!]
	\centering
	%\makebox[\textwidth]
%	{
	    	\includegraphics[width=0.9\textwidth,height=5.5cm]{figures/hla.png}
%	}
%
	\caption{The Data architecture of the AQSS case study - (HLA)}
	\label{fig:ndr-hla}
    \end{figure*}
\end{center}
%Figure \ref{fig:ndr-hla} shows the High Level Architecture (HLA) for the case study, which describe the case in one node and the elements inside the node to give abstract data view about the case without any details. 
%\todo[inline]{Or we expand this text, or we remove it. It does not make any sense to have only three lines about it!}
